Feedback Design and Implementation for Integrated Posture Manipulation and Thrust Vectoring

This MS thesis outlines my contributions to the closed loop control and system integration of two robotic platforms: 1) Aerobat, a flapping wing robot stabilized by air jets, and 2) Harpy, a bipedal robot equipped with dual thrusters. Both systems share a common theme of the integration of posture manipulation and thrust vectoring to achieve stability and controlled movement. For Aerobat, I developed the software and control architecture that enabled its first untethered flights. The control system combines flapping wing dynamics with multiple air jet stabilization to maintain roll, pitch and yaw stability. These results were published in the IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS). For Harpy, I implemented a closed-loop control framework that incorporates active thruster assisted frontal dynamics stabilization . My work led to preliminary untethered dynamic walking. This approach demonstrates how thrust assisted stability can enhance locomotion in legged robots which has not been explored before.

==> COE_MS_PhD_Template/Makefile <==
# ------------------------------------------------------------------------
# Makefile:
# ------------------------------------------------------------------------
# written by:	Gunar Schirner 
# External References:
#   http://kriemhild.uft.uni-bremen.de/viewvc/vim/Makefile.pdflatex
#   http://www.tex.ac.uk/tex-archive/help/uk-tex-faq/Makefile
# last update:	$id$
#
# Help screen (start every help line with #h)
#
#h make        builds ALL_REF
#h
#h make publish 
#h             publish the build output to HTML publish directory  
#h
# --- names --------------------------------------------------------------

PROJECT	=	thesis

SRCNAME	=	$(PROJECT)_SRC.tar.gz
BINNAME	=	$(PROJECT)_BIN.tar.gz
ORIG	=	

TMP	=	/tmp
# own name
MAKEF   =       Makefile

# path for automatic publishing, put into your public_html directory`
PUBLISH_PATH = /home/student/<studentName>/public_html/thesis
VERSION_FILE = svnRev.tex

# set automatically by hook script (Post commit hook)
# SVN_REPO_PATH 
# SVN_REV

# --- lists --------------------------------------------------------------

ALL	=	$(PROJECT).pdf



# auto use all *.tex file in the own and in pi directory as dependency input 
INCLUDE	:=	$(shell [ -d tex ] && echo tex/*.tex )

SOURCES =	$(PROJECT).tex	\
		$(INCLUDE)

#BIBFILES :=  macro/bib-strings.bib macro/IEEEabrv.bib $(shell [ -d bib ] && echo bib/*.bib )

FIGFILES =

PPTFILES =	

PRNFILES =

# auto use all *.eps files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first eps is added 
EPSFILES :=	$(shell [ -d fig ] && echo fig/*.eps) 


# auto use all *.pdf files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first pdf is added 
#PDFFIGS :=	$(shell [ -d fig ] && echo fig/*.pdf) 


FIGURES	=	$(EPSFILES:.eps=.pdf) $(PDFFIGS)

#MACROS	=	macro/macros.tex

OTHERS	=	Makefile	


ORIGS	=	$(SOURCES) $(MACROS) $(OTHERS)

SRCTAR	=	$(SOURCES) $(MACROS) $(OTHERS)	\
		$(FIGFILES) $(PPTFILES) $(PRNFILES) $(EPSFILES)

BINTAR	=	$(ALL)

# --- environment --------------------------------------------------------

TEXINPUTS =	TEXINPUTS=.:MACROS:

TEXENV	=	$(TEXINPUTS)

# --- commands -----------------------------------------------------------

FIGPS	=	fig2dev -L ps
PRN2EPS	=	PATH=bin:$$PATH prn2eps
LATEX	=	$(TEXENV) latex
PDFLATEX =      pdflatex --interaction nonstopmode
BIBTEX	=	bibtex
DVIPS	=	dvips -Z -D 600 -t letter -Ppdf
PS2PDF	=	ps2pdf
EPS2PDF	=	epstopdf
PSSEL	=	psselect
TAR	=	gtar cvzf
RM	=	rm -f
MV	=	mv -f
MAKEIDX	=	makeindex
GV	=	ghostview
ECHO	=	echo
GREP	=	grep
WC	=	wc
CD	=	cd
CAT	=	cat
XLESS	=	xless
SPELL	=	nspell -t
SORT	=	sort -f
MAKEIDX	=	makeindex
DISTILL =       GS_OPTIONS="-dAutoFilterColorImages=false \
                            -dColorImageFilter=/FlateEncode" ps2pdf14
THUMBPDF=       thumbpdf --modes=dvips

# parse string to cause rebuild of latex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right|Table widths have changed. Rerun LaTeX.|Linenumber reference failed)"

# parse string to cause rebuild of bibtex
RERUNBIB = "No file.*\.bbl|Citation.*undefined"



# --- general rules ------------------------------------------------------

.SUFFIXES:
.SUFFIXES:	.fig .ps .prn .eps .tex .bbl .pdf

.fig.ps:
	$(FIGPS) $*.fig $*.ps

.prn.eps:
	$(PRN2EPS) $*.prn $*.eps

#GS added automatic conversion for eps files, epstopdf packages seems
# not installed on this linux installation
.eps.pdf:
	$(EPS2PDF) $*.eps

.tex.bbl:
	$(LATEX) $*.tex
	$(BIBTEX) $*

# run pdflatex once and bib + subsequent pdflatex conditionally
%.pdf: %.tex
	$(PDFLATEX) $<
	@egrep -c $(RERUNBIB) $*.log && (bibtex $*;$(PDFLATEX) $<); true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true


# --- rules --------------------------------------------------------------

all:		$(ALL)

# automatically produce help message by grep for sepcial comment lines 
help:;	@sed -n -e 's/^#h//p'  < $(MAKEF) | sed -e 's/ALL_REF/$(ALL)/g'

# second phase of the publish requires to get the current SVN version 
ifdef SECOND_PHASE
SVN_REV := $(shell svn info | sed -n -e 's/.*Revision: //p')
endif

# debug rule to print current version 
echo_ver:
	@echo $(SVN_REV)

# paste the current version information into tex file so that it 
# can be included into build
create_version_file: 
	@echo "\\newcommand{\\svnRevRef}{$(SVN_REV)}" > $(VERSION_FILE)


# actual publishing action 
autobuild_publish_2nd: create_version_file
	make >  $(PUBLISH_PATH)/z_buildlog.r$(SVN_REV).log
	set -e ; for f in $(basename $(filter %.pdf, $(ALL))); do        \
		rm -f $(PUBLISH_PATH)/$$f.r*.pdf;                         \
		cp $$f.pdf $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf;   \
		rm -f $(PUBLISH_PATH)/$$f.pdf; \
		ln -s $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf $(PUBLISH_PATH)/$$f.pdf ;  \
	done

# if the revision is already passed in as a parameter, we do not 
# need to trieve it again 
ifneq ("$(SVN_REV)", "")
# clean update build and publish 
publish: clean svn_up autobuild_publish_2nd
else
# cleanup, svn update and kick off second phase
publish: 
	make clean
	svn up
	make autobuild_publish_2nd SECOND_PHASE=1
endif

# helper rule to call svn update 
svn_up: 
	svn up


clean:
	$(RM) $(ALL)
	$(RM) *.ps *.pdf
	$(RM) *.dvi
	$(RM) *.toc *.lot *.lof *.log *.aux
	$(RM) *.idx *.ind *.ilg
	$(RM) *.inx *.srt
	$(RM) *.blg *.bbl
	$(RM) *.out
	$(RM) *.BAK *.bak *~
	$(RM) macro/*.BAK macro/*.bak macro/*~
	$(RM) texput.log
	$(RM) $(ORIG)

tar:
	-$(MV) $(SRCNAME) $(SRCNAME).bak
	-$(MV) $(BINNAME) $(BINNAME).bak
	-$(TAR) $(SRCNAME) $(SRCTAR)
	-$(TAR) $(BINNAME) $(BINTAR)

spell:
	$(SPELL) $(SOURCES)

orig:	$(ORIG)

todo:	$(ORIG)
	-$(GREP) -n "\.\.\.\." `$(CAT) $(ORIG)` >$(TMP)/todo
	$(WC) -l $(TMP)/todo ; $(XLESS) $(TMP)/todo ; $(RM) $(TMP)/todo &

1:
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps

2:
	$(LATEX) $(PROJECT).tex
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps


# --- project rules ---

$(PROJECT).pdf:  $(PROJECT).tex $(MACROS) $(INCLUDE) $(FIGURES) $(BIBFILES) 


summary.pdf:	summary.tex

$(PROJECT).ps: $(PROJECT).pdf
	pdf2ps $<

Description.ps: $(PROJECT).ps
	$(PSSEL) 1-15 $(PROJECT).ps Description.ps

Description.pdf:	Description.ps
	$(DISTILL) Description.ps Description.pdf


References.ps: $(PROJECT).ps
	$(PSSEL) 16- $(PROJECT).ps References.ps

References.pdf:	References.ps
	$(DISTILL) References.ps References.pdf


# --- other rules ---

$(ORIG):	$(ORIGS)
	$(ECHO) >$(ORIG) $(ORIGS)



#h dbgPrint   VAR=<varName> print content of variable <varName>
dbgPrint:
	@echo "$(VAR)=$($(VAR))"
# --- EOF ----------------------------------------------------------------


==> COE_MS_PhD_Template/macro/macro.tex <==
% a set of default macros (outsourced of main document for cleanliness


\usepackage{amsfonts,amssymb,amsmath}			% special math characters
\usepackage{times}		% use Postscript fonts
\usepackage{bm}


% reference macros (capitals!)
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\chapref}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\lineref}[1]{line~\ref{#1}}
\newcommand{\Lineref}[1]{Line~\ref{#1}}

\newcommand{\ifyes}[1]{#1}
\newcommand{\ifno}[1]{}


% local macro
\usepackage{multirow}
\clubpenalty=1000
\widowpenalty=1000

% misc. settings
\setcounter{secnumdepth}{3}

% enable index generation
\makeindex
\usepackage{makeidx}
\usepackage{acronym}

% format URLs
\usepackage{url}
% default style was sf but it produced a too big font in the reference section
\urlstyle{tt}

% graphics package depending on backend driver
% are we directly producing pdf? ie. running pdflatex ?
\ifnum\pdfoutput>0
\usepackage[pdftex]{graphicx}
% enable on the fly conversion of eps figures when using pdfLatex
\usepackage{epstopdf}
\else
\usepackage{graphicx}
\fi


% ----------------------------------------------------------------- %
% hyperref to create bookmarks in the PDF for easier navigation


% either for pdflatex
\ifnum\pdfoutput>0
\usepackage[pdftex,%                    % hyper-references for ps2pdf
bookmarks=true,%                        % generate bookmarks ...
bookmarksnumbered=true,%                % ... with numbers
hypertexnames=false,%                   % needed for correct links to figures
breaklinks=true           %Allows link text to break across lines;
]{hyperref}
% or for dvips ..
\else
\usepackage[hypertex,%                  % hyper-references for ps2pdf
bookmarks=true,%                        % generate bookmarks ...
bookmarksnumbered=true,%                % ... with numbers
hypertexnames=false,%                   % needed for correct links to figures
breaklinks=true           %Allows link text to break across lines;
]{hyperref}
\fi


\hypersetup{				% setup PDF information fields
pdfauthor = {\authorRef},
pdftitle = {\titleRef},
pdfsubject = {\expandafter{\degreeRef} thesis submitted to Northeastern University},
pdfkeywords = {add keywords here}
pdfcreator = {LaTeX with hyperref package},
pdfproducer = {dvips + ps2pdf}}

\usepackage{microtype}


==> COE_MS_PhD_Template/tex/abstract.tex <==
% abstract.tex:

\begin{abstract}

This is a very abstract abstract.

\end{abstract}



==> COE_MS_PhD_Template/tex/acknowledgments.tex <==
% acknowledgements.tex:

\begin{acknowledgements}

Here I wish to thank those who have supported me during the process of the thesis work.... 
\end{acknowledgements}



==> COE_MS_PhD_Template/tex/acronyms.tex <==
% acronyms.tex

\chapter*{List of Acronyms}
\addcontentsline{toc}{chapter}{List of Acronyms}

% below is the list of acronym definitions, place them in alphabetical order
% since they will not be sorted again. 
\begin{acronym}
\acro{AHB}{Advanced High-performance Bus}.
	System bus definition within the AMBA 2.0 specification. Defines a high-performance bus including pipelined access, bursts, split and retry operations.

\acro{ATLM}{Arbitrated Transaction Level Model}.
  A model of a system in which communication is described as transactions, abstract of pins and wires.
  In addition to what is provided by the \acs{TLM}, it models arbitration on a bus transaction level.
\acro{TLM}{Transaction Level Model}.
  A model of a system in which communication is described as transactions, abstract of pins and wires.


\end{acronym}


==> COE_MS_PhD_Template/tex/conclusion.tex <==
\chapter{Conclusion}
\label{chap:conclude}

Writing a long manuscript is easy ... only if one starts early enough. 


==> COE_MS_PhD_Template/tex/dedication.tex <==
% dedication.tex:

\begin{dedication}
To my family.
\end{dedication}


==> COE_MS_PhD_Template/tex/intro.tex <==
% intro.tex:

\chapter{Introduction}
\label{chap:intro}
This is where the intro goes.
There is a planet ... where people still believe digital watches are the
greatest invention. It is mostly harmless.

\section{Life, Universe and Everything}
\label{chap:intro:design}

Simple, quantitative answers to the most pondering questions are beautiful. More about question of life, universe and everything can be found in \cite{book:42}.

This is where the text goes. One can refer to a previous chapter like \chapref{chap:intro}. To find all the other reference possibilities search in the MACROS folder for chapref. Also one can include pictures, preferably in the pdf format like shown in \figref{fig:intro:meth}. Graphics can also be included as eps, if graphics is in eps, the epstopdf packages converts it to pdf on the fly. See examples below in \figref{fig:intro:meth2}.

To keep the code clean, call all extra packages that you would like to use from the file macro.tex in the macro folder. Also keep all your graphics in the fig folder and all bibliography related files in the bib folder.

Make sure that you run bibtex and makeindex to geberate bibliography and index.

This demonstrates how to include a term\index{Term} into the index\index{Index}. For details, check out \cite{latex:index}.

\begin{figure}[htbp]
  \centering
    \includegraphics[width=0.5\textwidth]{fig/meth.pdf}
  \caption[Design methodology for SoC design]{\label{fig:intro:meth} Design methodology for SoC design (Source \cite{book:SpecC:yellow})}
\end{figure}

\begin{figure}[htbp]
  \centering
    \includegraphics[width=0.5\textwidth]{fig/meth.eps}
  \caption{\label{fig:intro:meth2} Design methodology but included as EPS figure}
\end{figure}

Also tables are possible as shown in \tabref{tab:ConclusionSummary}. What is really cool are the acronyms. The first time you use one, like \ac{TLM} then it appears with full description. Using it the second time makes only the acronym appears \ac{TLM}.

\begin{table}[htbp]
  \centering
     \begin{tabular}{|l|c|}
        \hline
         \textbf{Environment Condition} & \textbf{Applicable Model} \\
			\hline
			 \begin{tabular}{@{}l@{}}
			 $\bullet\,$ single master bus \\
			 $\bullet\,$ no overlap between masters bus access\\
			 \end{tabular}
			&
			 \ac{TLM}
			\\
			\hline
			 \begin{tabular}{@{}l@{}}
			 $\bullet\,$ only locked transfers \\
			 $\bullet\,$ unlocked transfers and low overlap\\
			 \end{tabular}
			&
			 \ac{ATLM}
			\\
			\hline
			 \begin{tabular}{@{}l@{}}
			 $\bullet\,$ unlocked transfers and high overlap\\
			 \end{tabular}
			&
			 bus functional
			\\
			\hline
		\end{tabular}
	\caption{Conclusion summary}
	\label{tab:ConclusionSummary}
\end{table}

Now time for some math\index{Math}:
\begin{align}
F(x)&=\int_{-\infty}^x f(u)\,du\\
\bm{Ax}&=\bm{b}\\
\mathbf{Ax}&=\mathbf{b}\\
\sin^2(\theta)+\cos^2(\theta)&=1\\
x&\in\mathcal{X}
\end{align}

The difference in using \verb1\bm1  and \verb1\mathbf1  is clear from above.
% --- EOF ---


==> tex/acronyms.tex <==
% acronyms.tex

\chapter*{List of Acronyms}
\addcontentsline{toc}{chapter}{List of Acronyms}

% below is the list of acronym definitions, place them in alphabetical order
% since they will not be sorted again. 
\begin{acronym}
\acro{BLDC}{Brushless DC (direct current) motor}.
	System bus definition within the AMBA 2.0 specification. Defines a high-performance bus including pipelined access, bursts, split and retry operations.

\acro{CAD}{Computer aided design}.

\acro{EDF}{Electric ducted fan}.
  A model of a system in which communication is described as transactions, abstract of pins and wires.
  In addition to what is provided by the, it models arbitration on a bus transaction level.
  
\acro{ESC}{Electronic speed controller}.
  A model of a system in which communication is described as transactions, abstract of pins and wires.
  
\acro{FDM}{Fusion deposition modeling}.
    System bus definition within the AMBA 2.0 specification. Defines a high-performance bus including pipelined access, bursts, split and retry operations.
    
\acro{PWM}{Pulse width modulation}.
    System bus definition within the AMBA 2.0 specification. Defines a high-performance bus including pipelined access, bursts, split and retry operations.


\end{acronym}


==> tex/dedication.tex <==
% dedication.tex:

\begin{dedication}
To my family.
\end{dedication}

